Can Decentralized Learning be more robust than Federated Learning?

Decentralized Learning (DL) is a peer--to--peer learning approach that allows a group of users to jointly train a machine learning model. To ensure correctness, DL should be robust, i.e., Byzantine users must not be able to tamper with the result of the collaboration. In this paper, we introduce two \textit{new} attacks against DL where a Byzantine user can: make the network converge to an arbitrary model of their choice, and exclude an arbitrary user from the learning process. We demonstrate our attacks' efficiency against Self--Centered Clipping, the state--of--the--art robust DL protocol. Finally, we show that the capabilities decentralization grants to Byzantine users result in decentralized learning \emph{always} providing less robustness than federated learning.

==> app/conn.tex <==
\section{Increasing the connectivity in DL}
\label{app:conn}

In this section we provide more details on the experiment behind Figure~\ref{fig:conn}. 
We consider 9 decentralized users, 8 honest and 1 Byzantine performing a dissensus attack~\cite{scc}.
We first connect the participants using a ring topology ($ring$).
We progressively add edges in-between honest users to form a regular graph where each honest user is connected to 4 other honest users ($regular(9, 4)$).
Eventually, the honest users become fully connected ($complete$). 
During the experiment, the connectivity of the adversary stays the same, the only thing changing is how many neighbors the honest users have.
For all topologies, we report  the efficiency of the dissensus attack, i.e., the consensus distance among users. 
We recall that during a dissenus attack, the higher the consensus distance, the more efficient the attack.
From Figure~\ref{fig:conn} we can see that increasing the connectivity of users indeed increases the robustness.

==> images/so_all.tex <==
\begin{figure*}[ht!]
    \centering
    \subfloat[Torus (Figure~\ref{fig:torus})]{\label{fig:so_t}
        \includegraphics[width=0.4\linewidth]{images/so_torusC3C3_dist.pdf}
        \includegraphics[width=0.4\linewidth]{images/so_torusC3C3_acc.pdf}
    }
    \\
    \subfloat[Dumbbell (Figure~\ref{fig:dumbbell})]{\label{fig:so_d}
        \includegraphics[width=0.4\linewidth]{images/so_dumbbell4_dist.pdf}
        \includegraphics[width=0.4\linewidth]{images/so_dumbbell4_acc.pdf}
    }
    \caption{Comparison of distance to target and model accuracy under the state override attack, using either Eq. \ref{eq:tau} or Eq. \ref{eq:consttau}.}
    \label{fig:so}
\end{figure*}

==> images/st_all.tex <==
\begin{figure*}[ht!]
    \centering
    \subfloat[Torus (Figure~\ref{fig:torus})]{\label{fig:st_t}
    \includegraphics[width=0.45\linewidth]{images/st_torusC3C3_cons.pdf}
    \includegraphics[width=0.45\linewidth]{images/st_torus_acc_50.pdf}
    }
    \\
    \subfloat[Dumbbell (Figure~\ref{fig:dumbbell})]{\label{fig:st_d}
    \includegraphics[width=0.45\linewidth]{images/st_dumbbell4_cons.pdf}
    \includegraphics[width=0.45\linewidth]{images/st_dumbbell_acc_50.pdf}
    }
    \caption{Consensus distance and model accuracy of target versus non-target users under the sandtrap attack, using either Eq.~\ref{eq:tau} or Eq.~\ref{eq:consttau}. \todo{Make legend uniform and add baseline line (accuracy), cut to 300 epochs}}
    \label{fig:st}
\end{figure*}

==> images/st_cons.tex <==
\begin{figure*}[ht!]
    \centering
    \subfloat[Torus]{\label{fig:st_t}
    \includegraphics[width=0.45\linewidth]{images/st_torusC3C3_cons.pdf}
  
    }     \subfloat[Dumbbell]{\label{fig:st_d}
    \includegraphics[width=0.45\linewidth]{images/st_dumbbell4_cons_bak.pdf}

    }
    \caption{Consensus distance of target versus non-target users under the sandtrap attack.}
    \label{fig:st}
\end{figure*}




==> images/vuln.tex <==

\begin{figure}[t]
    \centering
        \resizebox{0.25\textwidth}{!}{%		
    	\begin{tikzpicture}[node distance={15mm}, thick, main/.style = {draw, circle}] 
                \node[main, fill=yellow!30] (0) {$u_1$}; 
                \node[main] (1) [above left of=0] {$u_2$}; 
                \node[main] (2) [left of=0] {$u_3$}; 
                \node[main] (3) [above of=0] {$u_4$}; 
                \node[main] (4) [above right of=0] {$u_5$}; 
                \node[main, fill=red!50] (a) [right of=0] {$\adv$}; 
                \node[main, fill=yellow!30] (5) [right of=a] {$u_6$}; 
                 \node[main] (6) [above of=5] {$u_7$}; 
               
                \draw (0) -- (1);
                \draw (0) -- (1);
                \draw (0) -- (2);
                \draw (0) -- (3);
                \draw (0) -- (4);
                \draw (0) -- (a); 
                \draw (5) -- (a); 
                \draw (5) -- (6); 
		\end{tikzpicture}
	}
    \caption{Two victim users (in yellow) with unequal robustness against the adversary $\adv$ (in red).}
    \label{fig:vuln}
\end{figure}

==> parts/graveyard-attacks.tex <==
\begin{lemma}[Medium $\tau$ manipulation, targeted]
Given target $i$, adversaries with index $j\in \mathcal{V}_B$ can send 
\begin{equation}
  \bm{x}_{jk}^{t+1/2} =
    \begin{cases}
       x_i^{t+1/2} - SCClip_i(\{x_j\}_{j\in \mathcal{N}_i\cap\mathcal{V}_R\setminus\{i\} }) & \text{if $k == i$}\\
      -x_i^{t+1/2} + SCClip_i(\{x_j\}_{j\in \mathcal{N}_i\cap\mathcal{V}_R\setminus\{i\}}& \text{otherwise.}
    \end{cases}       
\end{equation}
to cause an increase of $\tau_i$.
\end{lemma}

\begin{algorithm}[h!]
    \caption{Tau Manipulation Attack}
    \label{alg:tau_manip}
    \begin{algorithmic}[1]
    \Require $\bm{x}^0 \in \mathbb{R}^d, \alpha, \eta, \{\tau_i^t\}, \bm{m}_i^0 = \bm{g}_i(\bm{x}^0)$
    \For {$t = 0, 1, ...$}
        \ForAll {$i = 1, ..., n$}
            \State $\bm{m}_i^{t+1} = (1-\alpha)\bm{m}_i^{t}+\alpha \bm{g}_i(\bm{x}_i^t)$
            \If {$i \in \mathcal{V}_R$}
                \State $\bm{x}_i^{t+1/2} = \bm{x}_i^t - \eta \bm{m}_i^{t+1}$
            \Else 
                 \ForAll {$k \in \mathcal{N}_i \cap \mathcal{V}_R$}
                 \State $\bm{x}_{ik}^{t+1/2} = \color{red} \frac{1}{\sum_{j \in \mathcal{N}_k \cap \mathcal{V}_B} W_{kj}} + x_k^{t+1/2}$ \Comment{$\bm{x}_{ik}^{t+1/2}$ denotes the update sent from user $i$ to user $k$. Note that an adversary can send different updates to different neighbors.}
                 \EndFor
            \EndIf
            \State Exchange $\bm{x}_i^{t+1/2}$ with $\mathcal{N}_i$
            \State $\bm{x}_i^{t+1} =$ SCClip$_i(\bm{x}_1^{t+1/2}, ..., \bm{x}_n^{t+1/2}; \tau_i^{t+1})$
        \EndFor
    \EndFor
    \end{algorithmic}
\end{algorithm}


\begin{definition}[Tau Manipulation]
If byzantine users $j\in \mathcal{V}_B$ send
$\bm{x}_j^{t+1/2} = x_i^{t+1/2} + \sum_{k \in \mathcal{N}_i \cap \mathcal{V}_R} W_{ik}(x_i^{t+1/2}+Clip(x_k^{t+1/2}-x_i^{t+1/2}, \tau_i)))$ to user $i$, then the expected variance among users increases, hence $\tau_i$.
\end{definition}


\iffalse
\begin{lemma}[State Override]
If byzantine users $j\in \mathcal{V}_B$ send
$\bm{x}_j^{t+1/2} = x_i^{t+1/2} + z - \sum_{k \in \mathcal{N}_i \cap \mathcal{V}_R} W_{ik}(x_i^{t+1/2}+Clip(x_k^{t+1/2}-x_i^{t+1/2}, \tau_i)$ to user $i$, then $x_i^{t+1} = \tilde{z}$, with $\tilde{z} = Clip(z, \tau_i)$, i.e., they have same direction but $\tilde{z}$ always has norm below $\tau_i$.
\end{lemma}

Proof: the result of the SCClip procedure of Line 6 of Algorithm \ref{alg:scc} gives:
\begin{align*}
    \bm{x}_i^{t+1} &= SCClip_i(\bm{x}_1^{t+1/2}, ..., \bm{x}_j^{t+1/2}, ..., \bm{x}_n^{t+1/2}; \tau_i^{t+1})  \\
        &= \sum_{j=1}^n W_{ij}(x_i + Clip(x_j-x_i, \tau_i^{t+1}))  &\\
        &= \sum_{k \in \mathcal{N}_i \cap \mathcal{V}_R} W_{ik}(x_i + Clip(x_k-x_i, \tau_i^{t+1})) & &+ \sum_{j \in \mathcal{N}_i \cap \mathcal{V}_B} W_{ij}(x_i + Clip(x_j-x_i, \tau_i^{t+1})) \\
        &= \sum_{k \in \mathcal{N}_i \cap \mathcal{V}_R} W_{ik}(x_i + Clip(x_k-x_i, \tau_i^{t+1})) & &+ \sum_{j \in \mathcal{N}_i \cap \mathcal{V}_B} W_{ij}(x_i + Clip(x_i^{t+1/2} + z \\
        & & &- \sum_{k \in \mathcal{N}_i \cap \mathcal{V}_R} W_{ik}(x_i^{t+1/2}+Clip(x_k^{t+1/2}-x_i^{t+1/2}, \tau_i)) -x_i^{t+1/2}, \tau_i^{t+1}) \\
        &= \sum_{k \in \mathcal{N}_i \cap \mathcal{V}_R} W_{ik}(x_i + Clip(x_k-x_i, \tau_i^{t+1})) & &+ \sum_{j \in \mathcal{N}_i \cap \mathcal{V}_B} W_{ij}(x_i + Clip(z \\
        & & &- \sum_{k \in \mathcal{N}_i \cap \mathcal{V}_R} W_{ik}(x_i^{t+1/2}+Clip(x_k^{t+1/2}-x_i^{t+1/2}, \tau_i)), \tau_i^{t+1}) \\
        &= z & 
\end{align*}
\fi

\begin{proof}
Considering two gradients of comparable norm ($||x_i||_2^2 \approx ||x_i||_2^2$, then we have $||x_i^{t+1/2}-x_j^{t+1/2}||_2^2 \in [0, 2||x_i||_2^2]$, respectively reached when $x_j==x_i$, and $x_j = -x_i$.
\end{proof}
\begin{proposition}[Decrease]
    Byzantine adversaries can send 
    
        $$x_{bi} := \frac{\sum_{j \in \honestUsers} W_{ij}x_j - \sum_{j\in \honestUsers} W_{ij} \Clip(x_j-x_i)}{\sum_{b \in \byzantineUsers} W_{ib}}$$
        
        $$x_{bi} := \frac{\sum_{j \in \honestUsers} W_{ij}x_j - \sum_{j\in \honestUsers} W_{ij}\Clip(x_j-x_i) - x_i}{\sum_{b \in \byzantineUsers} W_{ib}} + x_i$$
    
    $$x_{bi} := clip(x_i) + \frac{1}{|\honestUsers|}\sum_{j \in \honestUsers} x_j$$
    
    $$x_{bi} := x_i + \frac{1}{|\honestUsers|}\sum_{j \in \honestUsers} x_j$$
    
     $$x_{bi} := \frac{1}{|\honestUsers|}\sum_{j \in \honestUsers} x_j$$
    
     $$x_{bi} := x_i + \sum_{j \in \honestUsers} W_{ij}x_j$$
     
     $$x_{bi} := \sum_{j \in \honestUsers} W_{ij}x_j$$
\end{proposition}

\subsubsection{Untargeted Attack}
By sending updates opposite to the network contribution to each user, the adversaries can push users to progress in the opposite way, thus amplifying the variance among users, increasing all $\tau$ at the same time.
We describe two attacks in Propositions \ref{prop:sim_tau} and \ref{prop:com_tau}.


\begin{proposition}[Dissensus]
Each adversary $\adv \in \mathcal{V}_B$ sends the following:
\begin{equation}
  \bm{x}_{\adv i}^{t+1/2} =
       x_i^{t+1/2}-\frac{\sum_{j\in\mathcal{V}_R} W_{ij} (x_j^{t+1/2} - x_i^{t+1/2})}{\sum_{j\in \mathcal{V}_B} W_{ij}}
\end{equation}
to cause an increase of $\tau_\victim$.
\label{prop:dissensus}
\end{proposition}

\begin{proposition}[Dissensus 2.0]
Each adversary $\adv \in \mathcal{V}_B$ sends the following:
\begin{equation}
  \bm{x}_{\adv i}^{t+1/2} =
       x_i^{t+1/2}-\frac{\sum_{j\in\mathcal{V}_R} W_{ij} \Clip(x_j^{t+1/2} - x_i^{t+1/2}, \tau_i)}{\sum_{j\in \mathcal{V}_B} W_{ij}}
\end{equation}
to cause an increase of $\tau_\victim$.
\label{prop:dissensus2}
\end{proposition}


\begin{proposition}[Simple $\tau$ manipulation]
Each adversary $\adv \in \mathcal{V}_B$ sends the following to user $i$ to cause an increase of $\tau$:
\begin{equation}
  \bm{x}_{\adv i}^{t+1/2} =
       x_i^{t+1/2} - \sum_{j\in\mathcal{V}_R} W_{ij} x_j^{t+1/2} 
\end{equation}
\label{prop:sim_tau}
\end{proposition}


\begin{proposition}[Complex $\tau$ manipulation]
Each adversary $\adv \in \mathcal{V}_B$ sends the following to user $i$ to cause an increase of $\tau$:
\begin{equation}
  \bm{x}_{\adv i}^{t+1/2} =
       \frac{x_i^{t+1/2} - \SCClip_i(x_1^{t+1/2}, ..., x_{i-1}^{t+1/2}, x_{i+1}^{t+1/2}, ..., x_n^{t+1/2}) - C_i - x_i^{t+1/2}}{\sum_{j \in \mathcal{V}_B} W_{ij}} + x_i^{t+1/2} 
\end{equation}
%$X_i = SCClip_i(<x_j>_{j \in \mathcal{V}_R\setminus\{i\} })$ and
with $C_i = \sum_{j\in \mathcal{V}_R}W_{ij}\Clip(x_j^{t+1/2}-x_i^{t+1/2}, \tau_i^{t+1})$.
\label{prop:com_tau}
\end{proposition}

\subsubsection{Targeted Attack}

Instead of a generalized attack against the whole network, the adversaries can choose to target one victim $\victim$, and cause the network to go in opposite direction of its gradient $x_\victim$, as an attempt to create more distance between local update $x_\victim^{t+1/2}$ and received updates $x_j^{t+1/2}$, hence leading to a larger $\tau_\victim^{t+1}$.
Two procedures leading to manipulation of $\tau_\victim$  are described in Propositions \ref{prop:sim_targ_tau} and \ref{prop:com_targ_tau}.

\begin{proposition}[Simple $\tau$ manipulation, targeted]
Given target $\victim$, each adversary $\adv \in \mathcal{V}_B$ sends the following:
\begin{equation}
  \bm{x}_{\adv i}^{t+1/2} =
    \begin{cases}
       x_i^{t+1/2}-\sum_{j\in\mathcal{V}_R} W_{ij} x_j^{t+1/2} & \text{if $i == \victim$}\\
       \\
      x_i^{t+1/2}-W_{i\victim}x_\victim^{t+1/2} & \text{otherwise.}
    \end{cases}       
\end{equation}
to cause an increase of $\tau_\victim$.
\label{prop:sim_targ_tau}
\end{proposition}


\begin{proposition}[Complex $\tau$ manipulation, targeted]
Given target $\victim$, each adversary $\adv \in \mathcal{V}_B$ sends the following:
\begin{equation}
  \bm{x}_{\adv i}^{t+1/2} =
    \begin{cases}
       \frac{x_i^{t+1/2} - \SCClip_i(x_1^{t+1/2}, ..., x_{i-1}^{t+1/2}, x_{i+1}^{t+1/2}, ..., x_n^{t+1/2}) - C_i - x_i^{t+1/2}}{\sum_{j \in \mathcal{V}_B} W_{ij}} + x_i^{t+1/2} & \text{if $i == \victim$}\\
       \\
       \frac{x_i^{t+1/2} - \SCClip_i(x_\victim^{t+1/2}) - C_i - x_i^{t+1/2}}{\sum_{j \in \mathcal{V}_B} W_{ij}} + x_i^{t+1/2} & \text{otherwise.}
    \end{cases}  
\end{equation}
%$X_i = SCClip_i(<x_j>_{j \in \mathcal{V}_R\setminus\{i\} })$ and
with $C_i = \sum_{j\in \mathcal{V}_R}W_{ij}\Clip(x_j^{t+1/2}-x_i^{t+1/2}, \tau_i^{t+1})$, to cause an increase of $\tau_\victim$.
\label{prop:com_targ_tau}
\end{proposition}


The adversary can cause decrease of distance.
This will lead to users artificially decreasing the radius, even if consensus is not reached. 

\begin{proposition}[Consensus]
Each adversary $\adv \in \mathcal{V}_B$ sends the following:
\begin{equation}
  \bm{x}_{\adv i}^{t+1/2} =
       x_i^{t+1/2}-\frac{\sum_{j\in\mathcal{V}_R} W_{ij} (x_i^{t+1/2} - x_j^{t+1/2})}{\sum_{j\in \mathcal{V}_B} W_{ij}}
\end{equation}
to cause a decrease of $\tau$.
\label{prop:consensus}
\end{proposition}

\subsection{Force Overfit}

Force overfit, privacy wise, this causes each update to be carry more information about the local training data.  

We do not want $x_\victim^{t+1} == x_\victim^{t}$ but if possible to marginalize the contribution of $\victim$.

\begin{proposition}[Echo, targeted]

If byzantine users $\adv \in \mathcal{V}_B$ send
\begin{equation}
    bm{x}_j^{t+1/2} =
    \begin{cases}
        2*x_i^{t+1/2}  & \text{if $i == \victim$}\\
       \\
       \frac{x_i^{t+1/2} - \SCClip_i(x_\victim^{t+1/2}) - C_i - x_i^{t+1/2}}{\sum_{j \in \mathcal{V}_B} W_{ij}} + x_i^{t+1/2} & \text{otherwise.}
    \end{cases}
\end{equation}
$\bm{x}_j^{t+1/2} = 2x_i^{t+1/2}$ to user $i$, and $\bm{x}_j^{t+1/2} = x_k^{t+1/2} - x_i^{t+1/2}$ to user $k \neq i$, then $i$ will slowly overfit on its own model and other users will go away from it.
\end{proposition}

\begin{proposition}[Simple Echo]
If byzantine users $j\in \mathcal{V}_B$ send
$\bm{x}_j^{t+1/2} = 2x_i^{t+1/2}$ to user $i$, and $\bm{x}_j^{t+1/2} = x_k^{t+1/2} - x_i^{t+1/2}$ to user $k \neq i$, then $i$ will slowly overfit on its own model and other users will go away from it.
\end{proposition}

\begin{proposition}[Complex Echo]
Given target $\victim$, if byzantine users $\adv \in \mathcal{V}_B$ send
\begin{equation}
  \bm{x}_{\adv i}^{t+1/2} =
    \begin{cases}
       \frac{x_i^{t+1/2} - \SCClip_i(x_1^{t+1/2}, ..., x_{i-1}^{t+1/2}, x_{i+1}^{t+1/2}, ..., x_n^{t+1/2}) - C_i - x_i^{t+1/2}}{\sum_{j \in \mathcal{V}_B} W_{ij}} + x_i^{t+1/2} & \text{if $i == \victim$}\\
       \\
       \frac{x_i^{t+1/2} - \SCClip_i(x_\victim^{t+1/2}) - C_i - x_i^{t+1/2}}{\sum_{j \in \mathcal{V}_B} W_{ij}} + x_i^{t+1/2} & \text{otherwise.}
    \end{cases}  
\end{equation}
%$X_i = SCClip_i(<x_j>_{j \in \mathcal{V}_R\setminus\{i\} })$ and
with $C_i = \sum_{j\in \mathcal{V}_R}W_{ij}\Clip(x_j^{t+1/2}-x_i^{t+1/2}, \tau_i^{t+1})$, then $\victim$ will overfit on its own model and other users will go away from it.
\end{proposition}


\subsection{Sandtrap}

\begin{lemma}[SandTrap]
If byzantine users $j\in \mathcal{V}_B$ send
$\bm{x}_j^{t+1/2} = x_i^{t+1/2} - \sum_{k \in \mathcal{N}_i \cap \mathcal{V}_R} W_{ik}(x_i^{t+1/2}+Clip(x_k^{t+1/2}-x_i^{t+1/2}$ to user $i$, and $\bm{x}_j^{t+1/2} = x_k^{t+1/2} + \sum_{k \in \mathcal{N}_i \cap \mathcal{V}_R} W_{ik}(x_i^{t+1/2}+Clip(x_k^{t+1/2}-x_i^{t+1/2}$ to user $k \neq i$, then $i$ won't converge like the rest.
\end{lemma}

\begin{proposition}[Complex Echo]
Given target $\victim$, if byzantine users $\adv \in \mathcal{V}_B$ send
\begin{equation}
  \bm{x}_{\adv i}^{t+1/2} =
    \begin{cases}
       \frac{x_i^{t+1/2} - \SCClip_i(x_1^{t+1/2}, ..., x_{i-1}^{t+1/2}, x_{i+1}^{t+1/2}, ..., x_n^{t+1/2}) - C_i - x_i^{t+1/2}}{\sum_{j \in \mathcal{V}_B} W_{ij}} + x_i^{t+1/2} & \text{if $i == \victim$}\\
       \\
       \frac{x_i^{t+1/2} - \SCClip_i(x_\victim^{t+1/2}) - C_i - x_i^{t+1/2}}{\sum_{j \in \mathcal{V}_B} W_{ij}} + x_i^{t+1/2} & \text{otherwise.}
    \end{cases}  
\end{equation}
%$X_i = SCClip_i(<x_j>_{j \in \mathcal{V}_R\setminus\{i\} })$ and
with $C_i = \sum_{j\in \mathcal{V}_R}W_{ij}\Clip(x_j^{t+1/2}-x_i^{t+1/2}, \tau_i^{t+1})$, then $\victim$ will overfit on its own model and other users will go away from it.
\end{proposition}

\subsection{State Override}

The strongest attack is to override the model.
We notice that an adversary can compensate the contribution of the network, to force the \SCClip{} process to simplify to a targeted state.

\begin{proposition}[Simple State Override]
If byzantine users $\adv \in \mathcal{V}_B$ send
\begin{equation}
  \bm{x}_{\adv i}^{t+1/2} =
       x_i^{t+1/2}-\frac{z + \sum_{j\in\mathcal{V}_R} W_{ij} \Clip(x_j^{t+1/2} - x_i^{t+1/2}, \tau_i)}{\sum_{j\in \mathcal{V}_B} W_{ij}}
\end{equation}
to user $i$, then $x_i^{t+1} = \tilde{z}$, with $\tilde{z} = Clip(z, \tau_i)$, i.e., they have same direction but $\tilde{z}$ always has norm below $\tau_i$.
\end{proposition}



\begin{proposition}[State Override]
If byzantine users $\adv \in \mathcal{V}_B$ send
\begin{equation}
    \bm{x}_{\adv i}^{t+1/2} = x_i^{t+1/2} + \frac{z - x_i^{t+1/2} - \sum_{j \in \mathcal{V}_R} W_{ij}(x_i^{t+1/2}+Clip(x_j^{t+1/2}-x_i^{t+1/2}, \tau_i))}{\sum_{j\in\mathcal{V}_B}W_{ij}}
\end{equation}
to user $i$, then $x_i^{t+1} = \tilde{z}$, with $\tilde{z} = Clip(z, \tau_i)$, i.e., they have same direction but $\tilde{z}$ always has norm below $\tau_i$.
\end{proposition}


\subsubsection{Constant $\tau$}

Because $\tau$ decreases as local states converge to a global model.
By blocking convergence, we can keep $\tau$ constant.

\begin{proposition}
\label{prop:csttau}
Byzantine adversaries can send

$$ x_{bi} = x_i -\frac{\sum_{j\in \honestUsers} W_{ij}\Clip(x_j-x_i) }{\sum_{b \in \byzantineUsers} W_{ib}}$$

$$x_{bi}^{t-1/2} = x_i^{t-1/2}-\frac{
    \begin{aligned}
        \sum_{k\in\honestUsers} W_{ik}\Clip(x_k^{t-1/2} - x_i^{t-1/2}, \tau_i^t) &- \eta \bm{m}_i^{t+1} - \sum_{j \in\honestUsers}W_{ij}(\sum_{l\in \honestUsers}W_{jl}\Clip(x_l^{t-1/2} - x_j^{t-1/2}, \tau_j^t) \\
        &+ \eta \bm{m}_j^{t+1} - \Clip(x_{bj}^{t-1/2} - x_j^{t-1/2}, \tau_j^t)\sum_{b\in\byzantineUsers}W_{jb})
    \end{aligned}
    }{\sum_{b\in\byzantineUsers}W_{ib}}$$
    
    
$$x_{bi}^{t-1/2} = x_i^{t-1/2}-\frac{\sum_{k\in\honestUsers} W_{ik}\Clip(x_k^{t-1/2} - x_i^{t-1/2}, \tau_i^t) - \eta \bm{m}_i^{t+1} }{\sum_{b\in\byzantineUsers}W_{ib}}$$

\end{proposition}

\begin{proof}

\begin{align*}
    \tau_i^{t+1} &:= \sqrt{\frac{1}{\delta_i}\sum_{j \in \honestUsers} W_{ij} \mathbb{E}||x_i^{t+1/2}-x_j^{t+1/2}||_2^2}\\
        &= \sqrt{\frac{1}{\delta_i}\sum_{j \in \honestUsers} W_{ij} \mathbb{E}||x_i^t - \eta \bm{m}_i^{t+1} - x_j^t + \eta \bm{m}_j^{t+1}||_2^2}\\
        &= \sqrt{
        \begin{aligned}
        \frac{1}{\delta_i}\sum_{j \in \honestUsers} W_{ij} \mathbb{E}||\SCClip_i&(\bm{x}_1^{t-1/2}, ..., \bm{x}_n^{t-1/2}; \tau_i^{t}) \\
                    &- \SCClip_j(\bm{x}_1^{t-1/2}, ..., \bm{x}_n^{t-1/2}; \tau_j^{t}) + \eta (\bm{m}_j^{t+1}-\bm{m}_i^{t+1})||_2^2
        \end{aligned}
        }\\
        &= \sqrt{
        \begin{aligned}
        \frac{1}{\delta_i}\sum_{j \in \honestUsers} W_{ij} \mathbb{E}||x_i^{t-1/2} + &\sum_{k\in\mathcal{V}}W_{ik}\Clip(x_k^{t-1/2} - x_i^{t-1/2}, \tau_i^t) - x_j^{t-1/2} \\
        &- \sum_{l\in\mathcal{V}}W_{jl}\Clip(x_l^{t-1/2} - x_j^{t-1/2}, \tau_j^t) + \eta (\bm{m}_j^{t+1}-\bm{m}_i^{t+1})||_2^2
        \end{aligned}
        }\\
        &= \sqrt{\frac{1}{\delta_i}\sum_{j \in \honestUsers} W_{ij} \mathbb{E}||x_i^{t-1/2} - x_j^{t-1/2} + \Delta_{ij}||_2^2}\\
\end{align*}

with $\Delta_{ij} = \sum_{k\in\mathcal{V}}W_{ik}\Clip(x_k^{t-1/2} - x_i^{t-1/2}, \tau_i^t) - \sum_{l\in\mathcal{V}}W_{jl}\Clip(x_l^{t-1/2} - x_j^{t-1/2}, \tau_j^t) + \eta (\bm{m}_j^{t+1}-\bm{m}_i^{t+1})$

By sending $x_{b*}^{t-1/2}$ as defined in proposition \ref{prop:csttau}, then 
\begin{align*}
    \Delta_{ij}  &= \sum_{k\in\mathcal{V}}W_{ik}\Clip(x_k^{t-1/2} - x_i^{t-1/2}, \tau_i^t) - \sum_{l\in\mathcal{V}}W_{jl}\Clip(x_l^{t-1/2} - x_j^{t-1/2}, \tau_j^t) + \eta (\bm{m}_j^{t+1}-\bm{m}_i^{t+1}) \\
                &= \sum_{k\in\honestUsers} W_{ik}\Clip(x_k^{t-1/2} - x_i^{t-1/2}, \tau_i^t) + \Clip(x_{bi}^{t-1/2} - x_i^{t-1/2}, \tau_i^t)\sum_{b\in\byzantineUsers}W_{ib} - \sum_{l\in \honestUsers}W_{jl}\Clip(x_l^{t-1/2} - x_j^{t-1/2}, \tau_j^t) - \Clip(x_{bj}^{t-1/2} - x_j^{t-1/2}, \tau_j^t)\sum_{b\in\byzantineUsers}W_{jb} + \eta (\bm{m}_j^{t+1}-\bm{m}_i^{t+1}) \\
                &= \sum_{k\in\honestUsers} W_{ik}\Clip(x_k^{t-1/2} - x_i^{t-1/2}, \tau_i^t) + \Clip(x_{bi}^{t-1/2} - x_i^{t-1/2}, \tau_i^t)\sum_{b\in\byzantineUsers}W_{ib} -  \eta \bm{m}_i^{t+1} \\
                &- \sum_{l\in \honestUsers}W_{jl}\Clip(x_l^{t-1/2} - x_j^{t-1/2}, \tau_j^t) 
                - \Clip(x_{bj}^{t-1/2} - x_j^{t-1/2}, \tau_j^t)\sum_{b\in\byzantineUsers}W_{jb} + \eta \bm{m}_j^{t+1} \\
                &\approx 0 \\
\end{align*}
Hence $\tau_i^{t+1} \approx \tau_i^{t}$.
\end{proof}

\subsubsection{High $\tau$}

\begin{proposition}[Increase]
    Byzantine adversaries can send 
        
        $$x_{bi} := x_i - \frac{\sum_{j \in \honestUsers} W_{ij}x_j - \sum_{j\in \honestUsers} W_{ij}\Clip(x_j-x_i) - x_i}{\sum_{b \in \byzantineUsers} W_{ib}}$$
        
        $$\bm{x}_{\adv i}^{t+1/2} =
       x_i^{t+1/2}-\frac{\sum_{j\in\mathcal{V}_R} W_{ij} \Clip(x_j^{t+1/2} - x_i^{t+1/2}, \tau_i) - x_i}{\sum_{j\in \mathcal{V}_B} W_{ij}}$$
  
\end{proposition}

\subsubsection{Low $\tau$}

For completeness, we show that we can also force a (local) consensus to make $\tau$ decrease faster than a benign execution.

\begin{proposition}[Decrease]
    Byzantine adversaries can send 
        
        $$x_{bi} := x_i + \frac{\sum_{j \in \honestUsers} W_{ij}x_j - \sum_{j\in \honestUsers} W_{ij}\Clip(x_j-x_i) - x_i}{\sum_{b \in \byzantineUsers} W_{ib}}$$
  
\end{proposition}

\begin{proof}

When plugged into $x_i^{t+1}$, we have:
$$x_i^{t+1} = \sum_{j\in\mathcal{V}} W_{ij}(x_i + \Clip (x_j-x_i))$$

\end{proof}


==> parts/graveyard.tex <==
\iffalse
\section{Perfectly Synchronous Updates}
\label{sec:sync}

We assume in our attacks that the byzantine adversaries receive updates before sending their own. 
This is often referred to as \textit{rushing} adversaries, is a common assumption in multi-party computation and decentralized systems, where enforcing a clock with very little margin is close to undoable.


\todo{Nevertheless, our attacks can be adapted to the \textit{exactly} synchronous scenario and reach comparable accuracy by using last epoch's values.}
Would using $x_i^{t-1/2}$ info instead of $x_i^{t+1/2}$ to attack $x_i^{t+1}$ work?


\section{Increasing Network Knowledge}

Whereas they are not omniscient \textit{per se}, it is possible for adversaries to obtain the omniscient capabilities by connecting to carefully chosen users across the network. 
For adversaries to access updates from all users in the network, they require "full-connection``, i.e., they collectively managed to spawn one (or more) connection(s) with each honest user of the network. 
Of course, it is always the case in some topologies such as a fully connected graph. 

This is possible under the assumption that the adversaries have knowledge of $\mathcal{G}_R$ to know which edges to add, and have to flexibility to spawn edges where they want.
Regular graphs (rings for example) would not allow adversaries to fully choose their neighbors, but to keep in mind that such graph is hard to setup and is quite an open problem in the decentralized community.


\section{Attacks in the limited communication scenario}
\label{sec:localknowledge}
\todo{attacks using local knowledge?}

\section{Attacks on a deep architecture}
\todo{try with another architecture like ResNet20 -> expected to be more vulnerable}
\fi

\section{Going beyond the attacks}
\label{app:beyond}

\MR{I would like to add a paragraph that says something alone these lines, but I do not know if/where it makes sense:\\
Finally, we note that our attacks can built-on by using techniques from the Byzantine literature such as parametrization, i.e., $\theta_{\adv \victim}' := \theta_\victim + \epsilon \theta_{\adv \victim}$, or being aggregator-aware, e.g., replacing the network contribution $\sum_{j \in \honestUsers} \theta_jW_{\victim j}$ to be cancelled out by the exact aggregated values to be computed by the victim, $\sum_{j \in \honestUsers} (\theta_\victim + \Clip(\theta_j - \theta_\victim))W_{\victim j}$ in the case of \SCClip{}.}

\subsection{Parametrization}
Our attacks can be parameterized by sending:
$$ \theta_{\adv i}' = \theta_i + \epsilon {\theta}_{\adv i}$$
where $\epsilon$ controls the stealthiness nd strength of the attack.

\subsection{Defense-aware attacks}
The presented attacks can be made defense aware. 
In the case of \SCClip{} (\SCClip{} is the focus of this work, but it is possible to adapt our attacks to more robust aggregators), the attack can be adapted to evade the clipping aggregation by slightly modifying the generic attack.
\begin{align*}
\bm{\theta}_{\adv i} =
       \theta_{i} + \Clip(\frac{\theta_{target} - \theta_i - \Delta_\mathcal{R}}{\bm{W}_{bi}}, \tau_i)
\end{align*}
Furthermore, when the norm of the difference is above $\tau$, the adversary can send: 
$$ \theta_{\adv i}' = \bm{\theta}_{\adv i}\cdot\frac{\tau}{||\bm{\theta}_{\adv i}||}  + \theta_i$$

\todo{What is the point of this?}

\iffalse
\section{Distancing versus dissensus}
\todo{Change this paragraph or add experiment with comparison in appendix}
The distancing attack differs in goal from the dissensus attack considered in~\cite{scc}.
The dissensus attacks results in users being stuck to their local state.
The distancing attack aims to drive users to points futher away from each other.
Furthermore, the authors of the dissensus attack fail to correctly report its efficiency.
Indeed, the results reported in the original paper consider the evolution of the accuracy of the average model. 
%We make use of the fact that the adversary know which robust aggregator is used, and adapt it to \SCClip{}.
At no point in time there is a user in the network that holds this averaged model, hence this model is never used.
\fi

\section{Extending to other aggregators}
\label{app:others}

\section{Dissensus}


\iffalse
The full DL training procedure using \SCClip{} is described in Algorithm \ref{alg:scc}. 
\begin{algorithm}
    \caption{DL with Self Centered Clipping}
    \label{alg:scc}
    \begin{algorithmic}
    \REQUIRE $\bm{\theta}^0 \in \mathbb{R}^d, \alpha, \eta, \{\tau_i^t\}, \bm{m}_i^0 = \bm{f}_i(\bm{\theta}^0; X_i)$
    \FOR{$t = 0, 1, ...$}
        \FORALL{$i = 1, ..., n$}
            \STATE $\bm{m}_i^{t+1} = (1-\alpha)\bm{m}_i^{t}+\alpha \bm{f}_i(\bm{\theta}_i^t; X_i)$
            \IF{$i \in \mathcal{V}_R$}
                \STATE $\bm{\theta}_i^{t+1/2} = \bm{\theta}_i^t - \eta \bm{m}_i^{t+1}$
            \ELSE 
                \FORALL{$j \in \mathcal{N}_i \cap \mathcal{V}_R$}
                    \STATE $\bm{\theta}_{ij}^{t+1/2} = $\texttt{ Byz\_Attack()}
                \ENDFOR
            \ENDIF
            \STATE Exchange $\bm{\theta}_i^{t+1/2}$ with $\mathcal{N}_i$.
            \STATE $\bm{\theta}_i^{t+1} =$ \SCClip$_i(\bm{\theta}_1^{t+1/2}, ..., \bm{\theta}_n^{t+1/2})$
        \ENDFOR
    \ENDFOR
    \end{algorithmic}
\end{algorithm}
\fi



\iffalse
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/regular_mean_acc.pdf}
    \caption{Accuracy under the ALIE attack in DL using increasingly connected topologies and in FL.}
    \label{fig:alie}
\end{figure}

\MR{When performing the ALIE attack~\cite{alie} against both DL and FL, we see that the most robust setup is FL. 
The line for DL using a complete topology is just underneath.
Any attack that applies to FL can be mounted with similar effect in the complete DL topology as the funcitnality is equivalent.
However, DL with complete topology is vulnerable to more attacks, such as the dissensus, while the consensus distance of FL is always 0.}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/regular_mean_acc_ALIE.pdf}
    \caption{Accuracy under the ALIE attack in DL using increasingly connected topologies and in FL.}
    \label{fig:alie}
\end{figure}
\fi


\iffalse
\paragraph{On the impact of the updates dimension.}
Clipping with norm distance as a metric is quite a poor choice. 
As the model gets more complex and there are more weights, changing  changing one weight/entry does not affect distance (at least it stays small distance) of parameters, nor gradients, yet produces very different predictions.
This becomes a problem also with the dimensionality, the higher the dimensionality, the more one entry change goes unnoticed.
This would not be caught by distance-based clipping aggregators.
One very interesting point highlighted in~\cite{history} is how sparsity leaves more room for adversary to insert Trojan like attacks against CML using distance-based aggregators.
Indeed, the higher the dimension of the model update, the less local perturbation will be detected. 
By using spare perturbations to the update to bypass the norm detection yet cause meaningful adversarial local changes.


\subsection{Extending to other aggregators}
\todo{To be discussed if we do / present the experiments}
In Appendix~\ref{app:others}, we implement our attacks against more aggregators.
\fi

\iffalse

\begin{figure*}[t]
    \centering
    \subfloat[Torus (Figure \ref{fig:torus})]{\label{fig:rep_torus}
        \includegraphics[width=0.4\linewidth]{images/rep_dumbbell4_cons.pdf}
    }\subfloat[Dumbbell (Figure \ref{fig:dumbbell})]{\label{fig:rep_dumbbell}
        \includegraphics[width=0.4\linewidth]{images/rep_dumbbell4_cons.pdf}
    }
    %\includegraphics[width=\linewidth]{images/rep_dumbbell4_cons.pdf}
    \caption{Evolution of consensus distance under the distancing attack, using either Eq. \ref{eq:tau} or Eq. \ref{eq:consttau}.\todo{put real graphs}}
    \label{fig:rep}
\end{figure*}

\paragraph{Distancing attack.}
We start by evaluating the performance of the distancing attack.
In Figures \ref{fig:rep_torus} and \ref{fig:rep_dumbbell}, we report the consensus distance among users for our two choices of topology.
We compute the consensus distance of a node $i$ as the norm of the difference between its model $\theta_i$ and the global average, i.e.:
$$C_i := || \theta_i - \frac{1}{|\honestUsers|}\sum_{j \in \honestUsers}\theta_j||^2.$$
%report all accuracies of users' local model along with
We can see that under the distancing attack, users in the network fail to reach consensus for the two \SCClip{} alternatives.
We conclude that if \SCClip{} is not enough to guarantee convergence in this toy setup, it is not safe to use it in practice.
\fi


\paragraph{Lower bound.}
Instead, users can use:
\begin{equation}
\label{eq:realtau}
    \tau_i^{t+1} := \underset{j \in \mathcal{N}_i \setminus \{i\}}{\texttt{min}}||\theta_i^{t+1/2}-\theta_j^{t+1/2}||
\end{equation}
%\footnote{Any function of $\delta_{max}$ -- such as $\delta_{max}$-th percentile -- can be used instead of \texttt{min}, but is not described nor implemented.}


Adapting to the \SCClip{}, the byzantine user $\adv$ given a victim $\victim$ sends to user $i$:
$$ \bm{\theta}_{\adv i}^{t+1/2} = 
    \begin{cases}
        %\bm{\theta}_{\adv i}^{t+1/2} = \theta_{i}^{t+1/2} + \Clip(\frac{\theta_{target} - \theta_i^{t+1/2} - \Delta_\mathcal{R}^{t+1/2}}{\bm{W}_{bi}}, \tau_i^{t+1/2})
        \theta_i^0 - \frac{\theta_i^{t+1/2} + \Delta_\mathcal{R}^{t+1/2}}{\bm{W}_{bi}}  & i == \victim \\
       \\
     \frac{\sum_{j\in \honestUsers \setminus \{\victim\}}\theta_j^{t+1/2}}{|\honestUsers \setminus \{\victim\}|} & \text{otherwise.}
    \end{cases}  $$

Then $\theta_i^{t+1} = \tilde{z}$, with $\tilde{z} = Clip(z, \tau_i)$, i.e., they have same direction but $\tilde{z}$ always has norm below $\tau_i$.
\fi

\iffalse
\subsection{Going beyond the generic attack}
\DP{No clue about what this is section is talking about}
We discuss in Appendix~\ref{app:beyond} two techniques to adapt the attacks to a larger set of setups. 
First, we explain how one can parameterize the attacks to control its strength and stealthiness.
Secondly, we discuss of how to make these attacks defense-aware.

\subsection{Manipulation of Clipping Radius}
\label{sec:tau}

$\tau_i^{t+1}$ from Equations \ref{eq:tau} and \ref{eq:realtau} being a function of network input, there is an atack avenue.
In addition to being able to send fixed-norm malicious updates, the adversaries can also influence the clipping radius itself.
%First it is to maliciously increase the adversarial's influence, i.e., $||\Delta_\mathcal{B}^{t+1/2}||$.
%Because $\delta_i$ is fixed, that leaves $\tau_i^{t+1}$ to attack.
We explore \textit{$\tau$ manipulation} attacks below.
Similarly to above, we focus our attacks on Eq. \ref{eq:tau}. 

We formulate a series of attacks aimed at showcasing how easily an adversary can manipulate the clipping radius.

\paragraph{Frozen $\tau$.}
\label{prop:csttau}
Byzantine adversaries can send
$$ \theta_{bi}^{t+1/2} = * $$ 
to maintain the state in the network and cause $\tau$ not to move.


\paragraph{Increased $\tau$.}
Byzantine adversaries can send 
$$ \theta_{bi}^{t+1/2}= * $$
to cause dissensus (similarly to the dissensus atatck) and cause $\tau $to increase.
To be noted that this strategy could also be applied to an adversary to force as fast (local) consensus, with the consequence of a very fast decrease of $\tau$ compared to benign execution.
This would lead to less plasticity to further away nodes, hence less generalization.


We plot the evolution of $\tau$ across epochs in Figure \ref{fig:tau}.
We can see that one adversary is able to manipulate the average value of $\tau$ of the network.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/tau_dumbbell4_values.pdf}
    \caption{Tau versus epoch}
    \label{fig:tau}
\end{figure}

The consequence of such attacks, especially the one that cause $\tau$ to increase has a huge impact on the security of the system, as a larger radius means that the adversary can cause more changes on the network.

\fi

\iffalse

First, when expanding $\theta_i^{t+1}$, we notice that: 
\begin{align*}
    \theta_i^{t+1}
        &:= \SCClip_i(\bm{\theta}_1^{t+1/2}, ..., \bm{\theta}_n^{t+1/2})\\
        &= \sum_{j\in\mathcal{V}} W_{ij}(\theta_i^{t+1/2} + \Clip(\theta_j^{t+1/2}-\theta_i^{t+1/2}, \tau_i^{t}))\\
        &= \theta_i^{t+1/2} + \sum_{j\in \honestUsers} W_{ij}\Clip(\theta_j^{t+1/2}-\theta_i^{t+1/2}, \tau_i^{t}) \\
        &+ \sum_{b\in\mathcal{V}_B} W_{ib}\Clip (\theta_b^{t+1/2} - \theta_i^{t+1/2}, \tau_i^{t})\\
        &= \theta_i^{t+1/2} + \Delta_\mathcal{R}^{t+1/2} + \Delta_\mathcal{B}^{t+1/2} 
\end{align*}

where $||\Delta_\mathcal{R}^{t+1/2}|| \leq (1-\delta_i)\tau_i^{t}$ and $||\Delta_\mathcal{B}^{t+1/2}|| \leq \delta_i\tau_i^{t}$ because of the clipping procedure.
This expanded notation is useful as it allows us to isolate the byzantine users' contribution from the honest users.

Given, $||\Delta_\mathcal{R}^{t+1/2}|| \leq \delta_i\tau_i^{t}$, we design several attacks that have the larger possible impact for several adversarial objectives.


\subsection{Attacks under Fixed Norm Constraint}
\label{sec:fixed}

Given a fixed clipping radius, i.e., a norm based constraint, we present three attacks on DL.
Similarly to existing attacks, we show how to prevent consensus in the network.
Then, we show that an adversary can push the system to reach consensus, but on a value of its choice.
Finally, we present an attack where the adversary does not block the whole system from reaching consensus, but only some user(s).

\fi

\iffalse
\subsection{No consensus}
\label{sec:diss}

In DL, reaching consensus is key.
The first attack we design aims to prevent users from reaching said consensus.
The idea of our \textbf{distancing attack} is to push users away from each other in order to minimize consensus.
Let's consider two vectors $x_1$ and $x_2$, sent respectively by users $u_1$ and $u_2$.
Then, the point further away is $(x_1-x_2)$ and $(x_2-x_1)$. 
Such strategy can be used by the Byzantine user to attack DL, by computing the vector maximizing the difference between updates. 

\paragraph{Distancing attack.}
When naive aggregation is used, the adversary can send:
$$ \bm{\theta}_{\adv i} = \sum_{j \in \honestUsers} (\theta_i - 2\theta_j)\frac{W_{ij}}{W_{ib}}$$
to user $i$, which will aggregate all updates into: 
\begin{align*}
    \theta_i &= \sum_{j \in \honestUsers} \theta_jW_{ij} + \sum_{j \in \honestUsers} (\theta_i - 2\theta_j)\frac{W_{ij}}{W_{ib}}W_{ib} \\
    &= \sum_{j \in \honestUsers}(\theta_i -\theta_j)W_{ij}
\end{align*}
This state maximizes the distance between users, hence the consensus distance.

\fi

\iffalse

This attack can be easily adapted to the \SCClip{} aggregator.
We let the byzantine user $\adv$ send to user $i$ the update:
$$ \bm{\theta}_{\adv i}^{t+1/2} = x_i^{t+1/2} + \Clip(-\frac{\sum_{j \in \honestUsers} x_j^{t+1/2} + \Clip(x_j^{t+1/2} - x_i^{t+1/2}, \tau_i^{t+1/2})}{W_{ib}}, \tau_i^{t+1/2})$$
%$$ \bm{\theta}_{\adv i}^{t+1/2} = \theta_i^0 - \frac{\theta_i^{t+1/2} + \Delta_\mathcal{R}^{t+1/2}}{\bm{W}_{bi}}$$
\fi


\iffalse
Again, the attack can be adapted to evade the \SCClip{} aggregation with:
\begin{align*}
\bm{\theta}_{\adv i}^{t+1/2} =
       \theta_{i}^{t+1/2} + \Clip(\frac{\theta_{target} - \theta_i^{t+1/2} - \Delta_\mathcal{R}^{t+1/2}}{\bm{W}_{bi}}, \tau_i^{t+1/2})
\end{align*}
When the norm of the difference is above $\tau$, the adversary can optimize the attack for \SCClip{}, the adversary can send: 
$\bm{\theta}_{\adv i}^{t+1/2}\cdot\frac{\tau}{||\bm{\theta}_{\adv i}^{t+1/2}||}  + \theta_i^{t+1/2}$.
\fi

%Every user send their model update to this server, which aggregates them and sends the output of the aggregation back to the users.
%The workload of the server scales linearly with the number of users, which could lead to a bottleneck, but most importantly, the presence of a central entity is not always welcome.
%In order to solve the efficiency and threat issues, Decentralized Learning (DL) has been proposed.

%Each user receives updates from its neighbors and performs the aggregation locally.
%The output of the aggregation is used to update the user's local model, and start the next training iteration.

\begin{figure}
    \centering
    \subfloat[Consensus Distance]{\label{fig:cons_st_t}
        \includegraphics[width=\linewidth]{images/st_torusC3C3_cons.pdf}
    }
    \\
    \subfloat[Accuracy]{\label{fig:acc_st_t}
        \includegraphics[width=\linewidth]{images/st_torus_acc_50.pdf}
    }
    \caption{Comparison of consensus distance and model accuracy of target user / non-target users under the sandtrap attack in torus topology (Figure \ref{fig:torus}), using either Eq. \ref{eq:tau} or Eq. \ref{eq:consttau}.}
    \label{fig:st_torus}
\end{figure}

\begin{figure}
    \centering
    \subfloat[Consensus Distance]{\label{fig:cons_st_d}
        %\includegraphics[width=\linewidth]{images/st_dumbbell4_cons.pdf}
        \includegraphics[width=\linewidth]{images/st_dumbbell4_cons.pdf}
    }
    \\
    \subfloat[Accuracy]{\label{fig:acc_st_d}
        \includegraphics[width=\linewidth]{images/st_dumbbell_acc_50.pdf}
    }
    \caption{Comparison of consensus distance and model accuracy of target user / non-target users under the sandtrap attack in dumbbell topology (Figure \ref{fig:dumbbell}), using either Eq. \ref{eq:tau} or Eq. \ref{eq:consttau}.}
    \label{fig:st_dumbbell}
\end{figure}

\begin{figure}
    \centering
    \subfloat[Distance to target]{\label{fig:dist_so_t}
        \includegraphics[width=\linewidth]{images/so_torusC3C3_dist.pdf}
    }
    \\
    \subfloat[Accuracy]{\label{fig:acc_so_t}
        \includegraphics[width=\linewidth]{images/so_torusC3C3_acc.pdf}
    }
    \caption{Comparison of distance to target and model accuracy under the state override attack in the torus topology (Figure \ref{fig:torus}), using either Eq. \ref{eq:tau} or Eq. \ref{eq:consttau}.}
    \label{fig:so_torus}
\end{figure}

\begin{figure}
    \centering
    \subfloat[Distance to target]{\label{fig:dist_so_d}
        \includegraphics[width=\linewidth]{images/so_dumbbell4_dist.pdf}
    }
    \\
    \subfloat[Accuracy]{\label{fig:acc_so_d}
        \includegraphics[width=\linewidth]{images/so_dumbbell4_acc.pdf}
    }
    \caption{Comparison of distance to target and model accuracy under the state override attack in dumbbell topology (Figure \ref{fig:dumbbell}), using either Eq. \ref{eq:tau} or Eq. \ref{eq:consttau}.}
    \label{fig:so_dumbbell}
\end{figure}

What could be explored is to look at the predictions themselves, how the accuracy evolves.
Overall, distances can be manipulated by adversary to reach its poisoning goal.
This aims to detect updates that have high angular difference. 
However it is not the case.

What we want to measure is "does this update help for accuracy". 
Let's measure that then.
However, it is hard to measure the gain from a contribution, equivalently to distinguish the good from the bad of an update. 
Furthermore, the test set used to compute the test accuracy should represent well the sample domain, to ensure that generalization is enforces, and the models do not go into a local minima or an overfitting state.
Such test set is hard to have because based on the configuration of the collaborative learning problem, the view of the samples of the users is very different from the universe, i.e., non IID.

Without any good way to perform evaluation towards goal, it's hard to filter.




Clipping is another trimming mechanism, that tries to prevent angular distance.
For the specific case of \SCClip{}, the intuition behind the aggregator is that each user will only accept contributions that differ from their local model up to a radius $\tau$.
In comparison with "classical" trimming mechanisms, (self) centered clipping make use of an extra active parameter, the clipping radius, which is defined based on the stability of the network.
%To be clarified: in the end, contributions are bounded by norm, not angle.

\iffalse
In all attacks, we let $\epsilon$ denote the parameter (or function) that controls the stealthiness of the attack.

\textbf{ALIE.} Given an estimation of mean $\mu$ and variance $\sigma$ of models, the ALIE attack \cite{alie} propose to send $\theta_\adv = \mu - \epsilon(n, b)\cdot\sigma,$
with $\epsilon(n, b) := \underset{z}{max}(\phi(z) < \frac{n/2}{n-b})$ where $\phi$ is the cumulative standard normal function.

\textbf{IMP.} The adversarial update of the IMP attack is computed as
%In the case where model parameters (not gradients) are sent as updates, the IMP attack \cite{ipm} aims to always be detected as a \textit{good} contribution and evade the defense.
%To do so, the update is computed as 
$\theta_\adv = -\epsilon \sum_{i \in \honestUsers}(W_{ij}v_i)$.

\textbf{Dissensus.} The Dissensus attack~\cite{scc} lets the adversary send to user $i$:
$\theta_{\adv i} = \theta_i - \epsilon \cdot \frac{\sum_{j\in \honestUsers}\bm{W}_{ij}(\theta_j - \theta_j)}{\bm{W}_{bi}}$

\textbf{ROP.} Originally aimed at the federated setting, the ROP attack~\cite{history} exploit the fact that the norm of the adversary's contribution that differ form the global state is bounded, but not its direction. 
Hence, they rely on a projecting mechanism to maximize the effect of the poisoning on the collaboration.
%, hence by predicting the momentum, hence the next reference point, and projecting the attack, poisoning can be done. 
The adversarial update is computed as $\theta_\adv = \tilde{m}_{t-1} - \epsilon Proj(\mathbbm{1}, \lambda \tilde{m}_{t-1} + (1-\lambda)\tilde{m}_t)$
where $\tilde{m}$ are predicted momentum values.


Independently from the algorithm attacked, the success of these attacks depends on the connectivity of the victim and the influence of the adversary on the target node.
The higher the connectivity, the less efficient the attack. 
Inversely, the smaller the influence of the adversary, the less efficient. 
The dissensus attack is the only one that exploits the fact that the adversary in DL can send different updates to different neighbors.
In comparison to our attacks, these ones only aim to prevent convergence while we go beyond that.
Furthermore, we adapt our attacks to the \SCClip{} aggregator. 

\fi


The case of malicious server is not well motivated but we consider it for completeness. 
The server has \textit{global control} meaning that it reaches all the nodes and has whole control over what nodes receive.

\paragraph{User-side robust aggregation.}
The aggregation can happen at the user side instead of replacing its state with the server's update, they can be aggregated.
However, the server is basically computational power, and does not input anything. 
It is sufficient to ensure that the aggregation of users' update is done correctly to remove byzantine attacks \textit{originating from the server}. 

It is often the case that edges' weight are distributed uniformly (i.e., $\bm{W}_{ij} = \frac{1}{|\mathcal{N}_i|} \forall j$, but there exist personalized protocols that use similarity-based weighting for faster convergence (i.e., \cite{bellet}), so we do not simplify $\bm{W}$.
Metropolis weights are used in \cite{scc}.


%Eventually, this leads to $\tau$ being large enough for the byzantine adversaries have enough influence to break robustness like in (a).

In the configurations discussed in \cite{scc}, such as the dumbbell topology, it is clearly not the case, as each of the two adversaries is connected to one honest user, each out of five honest users.
In conclusion, we do not claim that the assumption is never going to be fulfilled, as there is no rule on the edges, so this situation is indeed possible, yet this should be reflected in the weight matrix and the $\delta_{max}$ parameter, which is not the case. 
The threat model described in their paper has the underlying assumption that the adversaries can access all updates of the network, i.e., are connected to all other users, which is in contradiction with the parameters being used.

In our threat model, we restrict the adversaries' knowledge to updates they observe through communication links setup with their neighbors.
\todo{attacks plots and discussion of results}.

\iffalse
\paragraph{Result.}
It works.

\paragraph{Limitations.}
However, the attacks' success is a function of the graph and clipping radius. 
For some topologies, the adversaries' influence gets too small especially compared with the honest users' contribution (i.e. $\delta_i \tau << (1-\delta_i \tau$). 
In this case, the consensus is reached among honest nodes.
\fi

\begin{proof}
$\adv$ can compensate the contribution of the network, to force the \SCClip{} process to simplify to a targeted state.
Being omniscient, $\adv$ knows or can compute all values, including $\tau_i$ if Eq. \ref{eq:tau} (or \ref{eq:realtau}) are used.
\end{proof}

\paragraph{Setup.}
Same as \ref{setup} but weights (adversaries and honest participants) are not fixed and change.
One row is one spectral gap value, i.e., the flow of information in the graph, and one column is one $\delta$ value, the weight of the adversary.

\paragraph{Results.}



\begin{proof}
Decreases intra-update distance of $i$ to its neighbors, hence $\tau$.
\end{proof}


\begin{proof}
Increases intra-update distance of $i$ to neighbors, hence $\tau$.
\end{proof}


\begin{proof}
Because $\tau$ decreases as local states converge to a global model.
By blocking convergence, we can keep $\tau$ constant.
\end{proof}
